Contrastive Learning for Enhancing Robust Scene Transfer in Vision-based Agile Flight

Scene transfer for vision-based mobile robotics applications is a highly relevant and challenging problem. The utility of a robot greatly depends on its ability to perform a task in the real world, outside of a well-controlled lab environment. Existing scene transfer end-to-end policy learning approaches often suffer from poor sample efficiency or limited generalization capabilities, making them unsuitable for mobile robotics applications. This work proposes an adaptive multi-pair contrastive learning strategy for visual representation learning that enables zero-shot scene transfer and real-world deployment. Control policies relying on the embedding are able to operate in unseen environments without the need for finetuning in the deployment environment. We demonstrate the performance of our approach on the task of agile, vision-based quadrotor flight. Extensive simulation and real-world experiments demonstrate that our approach successfully generalizes beyond the training domain and outperforms all baselines.

==> data/InterConsistency_Data.tex <==
\addplot+[mark=*,
  boxplot prepared={
    lower whisker = 0.444482,
    lower quartile = 0.590637,
    median = 0.651126,
    upper quartile = 0.710130,
    upper whisker = 0.864174,
  }
] coordinates {
};
\addlegendentry{Finetuned AE};
\node at (axis cs:1.000000,0.000000) [text width = 0.8cm, align=center,anchor=south, font=\tiny] {0.65 \\0.12};

\addplot+[mark=*,
  boxplot prepared={
    lower whisker = 0.536645,
    lower quartile = 0.712485,
    median = 0.785196,
    upper quartile = 0.852163,
    upper whisker = 0.939919,
  }
] coordinates {
};
\addlegendentry{Aug CL};
\node at (axis cs:2.000000,0.000000) [text width = 0.8cm, align=center,anchor=south, font=\tiny] {0.78 \\0.14};

\addplot+[mark=*,
  boxplot prepared={
    lower whisker = 0.613303,
    lower quartile = 0.792777,
    median = 0.851496,
    upper quartile = 0.913572,
    upper whisker = 0.989837,
  }
] coordinates {
(9.000000,0.595000)
(9.000000,0.611000)
(9.000000,0.560000)
(9.000000,0.593000)
(9.000000,0.543000)
(9.000000,0.604000)
(9.000000,0.610000)
(9.000000,0.603000)
(9.000000,0.608000)
(9.000000,0.573000)
(9.000000,0.528000)
};
\addlegendentry{State CL};
\node at (axis cs:3.000000,0.000000) [text width = 0.8cm, align=center,anchor=south, font=\tiny] {0.84 \\0.12};

\addplot+[mark=*,
  boxplot prepared={
    lower whisker = 0.988393,
    lower quartile = 0.994115,
    median = 0.996613,
    upper quartile = 0.997936,
    upper whisker = 0.999595,
  }
] coordinates {
(1.000000,0.987000)
(1.000000,0.986000)
(1.000000,0.981000)
(1.000000,0.977000)
(1.000000,0.988000)
(1.000000,0.946000)
(1.000000,0.985000)
(1.000000,0.969000)
(1.000000,0.980000)
(1.000000,0.983000)
(1.000000,0.984000)
(1.000000,0.955000)
(1.000000,0.949000)
(1.000000,0.965000)
(1.000000,0.962000)
(1.000000,0.978000)
(1.000000,0.975000)
(1.000000,0.972000)
(1.000000,0.953000)
(1.000000,0.939000)
(1.000000,0.982000)
(1.000000,0.950000)
(1.000000,0.966000)
(1.000000,0.979000)
(1.000000,0.963000)
(1.000000,0.976000)
(1.000000,0.931000)
(1.000000,0.960000)
(1.000000,0.973000)
(1.000000,0.957000)
(1.000000,0.970000)
(1.000000,0.967000)
(1.000000,0.968000)
(1.000000,0.964000)
(1.000000,0.945000)
(1.000000,0.932000)
(1.000000,0.974000)
(1.000000,0.942000)
(1.000000,0.929000)
(1.000000,0.971000)
};
\addlegendentry{Ours};
\node at (axis cs:4.000000,0.000000) [text width = 0.8cm, align=center,anchor=south, font=\tiny] {\textbf{0.99} \\\textbf{0.00}};

\addplot+[mark=*,
  boxplot prepared={
    lower whisker = 0.860836,
    lower quartile = 0.912867,
    median = 0.932494,
    upper quartile = 0.948070,
    upper whisker = 0.982333,
  }
] coordinates {
(3.000000,0.844000)
(3.000000,0.846000)
(3.000000,0.824000)
(3.000000,0.849000)
(3.000000,0.859000)
(3.000000,0.850000)
(3.000000,0.855000)
(3.000000,0.834000)
(3.000000,0.857000)
(3.000000,0.842000)
(3.000000,0.856000)
(3.000000,0.840000)
(3.000000,0.811000)
(3.000000,0.837000)
(3.000000,0.821000)
(3.000000,0.853000)
(3.000000,0.847000)
(3.000000,0.831000)
(3.000000,0.815000)
(3.000000,0.828000)
(3.000000,0.860000)
(3.000000,0.841000)
(3.000000,0.825000)
(3.000000,0.812000)
(3.000000,0.822000)
(3.000000,0.854000)
(3.000000,0.838000)
(3.000000,0.851000)
(3.000000,0.848000)
(3.000000,0.845000)
(3.000000,0.829000)
(3.000000,0.784000)
(3.000000,0.858000)
(3.000000,0.843000)
(3.000000,0.839000)
(3.000000,0.836000)
(3.000000,0.852000)
};
\addlegendentry{CLIP ResNet};
\node at (axis cs:5.000000,0.000000) [text width = 0.8cm, align=center,anchor=south, font=\tiny] {0.93 \\0.04};

\addplot+[mark=*,
  boxplot prepared={
    lower whisker = 0.742217,
    lower quartile = 0.835495,
    median = 0.866879,
    upper quartile = 0.897783,
    upper whisker = 0.971088,
  }
] coordinates {
(2.000000,0.725000)
(2.000000,0.739000)
(2.000000,0.740000)
(2.000000,0.709000)
(2.000000,0.732000)
(2.000000,0.734000)
(2.000000,0.721000)
(2.000000,0.710000)
(2.000000,0.719000)
(2.000000,0.736000)
(2.000000,0.699000)
(2.000000,0.676000)
(2.000000,0.728000)
(2.000000,0.680000)
(2.000000,0.664000)
(2.000000,0.693000)
(2.000000,0.741000)
(2.000000,0.690000)
(2.000000,0.722000)
(2.000000,0.703000)
(2.000000,0.735000)
(2.000000,0.716000)
(2.000000,0.687000)
(2.000000,0.729000)
(2.000000,0.713000)
(2.000000,0.726000)
(2.000000,0.742000)
(2.000000,0.691000)
(2.000000,0.733000)
(2.000000,0.717000)
(2.000000,0.685000)
(2.000000,0.669000)
(2.000000,0.698000)
(2.000000,0.695000)
(2.000000,0.711000)
(2.000000,0.727000)
(2.000000,0.708000)
(2.000000,0.724000)
(2.000000,0.737000)
};
\addlegendentry{CLIP ViT};
\node at (axis cs:6.000000,0.000000) [text width = 0.8cm, align=center,anchor=south, font=\tiny] {0.87 \\0.06};

\addplot+[mark=*,
  boxplot prepared={
    lower whisker = 0.271060,
    lower quartile = 0.509298,
    median = 0.596279,
    upper quartile = 0.672633,
    upper whisker = 0.914962,
  }
] coordinates {
(7.000000,0.918634)
(7.000000,0.923487)
};
\addlegendentry{Dino v2};
\node at (axis cs:7.000000,0.000000) [text width = 0.8cm, align=center,anchor=south, font=\tiny] {0.60 \\0.16};

\addplot+[mark=*,
  boxplot prepared={
    lower whisker = 0.883035,
    lower quartile = 0.890902,
    median = 0.893443,
    upper quartile = 0.896151,
    upper whisker = 0.899165,
  }
] coordinates {
(4.000000,0.882000)
(4.000000,0.881000)
(4.000000,0.880000)
(4.000000,0.878000)
(4.000000,0.879000)
(4.000000,0.877000)
(4.000000,0.876000)
(4.000000,0.883000)
(4.000000,0.874000)
(4.000000,0.873000)
(4.000000,0.875000)
};
\addlegendentry{Masked AE};
\node at (axis cs:8.000000,0.000000) [text width = 0.8cm, align=center,anchor=south, font=\tiny] {0.89 \\0.01};

\addplot+[mark=*,
  boxplot prepared={
    lower whisker = 0.624022,
    lower quartile = 0.723044,
    median = 0.772165,
    upper quartile = 0.817132,
    upper whisker = 0.955527,
  }
] coordinates {
};
\addlegendentry{ResNet50};
\node at (axis cs:9.000000,0.000000) [text width = 0.8cm, align=center,anchor=south, font=\tiny] {0.78 \\0.09};



==> sections/acknowledgment.tex <==
\section{Acknowledgments} \label{sec:Acknowledgments}

==> sections/supplementary_material.tex <==
\section*{Supplementary Material}\label{sec:SupplementaryMaterial}
\textbf{Video: }\href{https://youtu.be/4A4YyPgEWD8}{https://youtu.be/4A4YyPgEWD8}


